On {\L}ukasiewicz Topological Semantics

In this paper, we propose fuzzy topological semantics for {\L}ukasiewicz valued modal logic, based on the standard {\L}ukasiewicz algebra. Within this setting, formulas are interpreted as fuzzy sets of truth values, while the modal operators are realized through fuzzy interior and closure operators. We define a Kripke-induced fuzzy Alexandroff topology and establish a precise correspondence between {\L}ukasiewicz fuzzy Kripke semantics and its topological counterpart. The proposed topological semantics validates the S4 modal axioms that include reflexivity, transitivity, monotonicity, normality, and the necessitation of truth.

==> eptcsdata.tex <==
\providecommand{\firstpage}{62}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.6}{10.4204/EPTCS.455.6}}

